Augmented Lagrangian Optimization under Fixed-Point Arithmetic

In this paper, we propose an inexact Augmented Lagrangian Method (ALM) for the optimization of convex and nonsmooth objective functions subject to linear equality constraints and box constraints where errors are due to fixed-point data. To prevent data overflow we also introduce a projection operation in the multiplier update. We analyze theoretically the proposed algorithm and provide convergence rate results and bounds on the accuracy of the optimal solution. Since iterative methods are often needed to solve the primal subproblem in ALM, we also propose an early stopping criterion that is simple to implement on embedded platforms, can be used for problems that are not strongly convex, and guarantees the precision of the primal update. To the best of our knowledge, this is the first fixed-point ALM that can handle non-smooth problems, data overflow, and can efficiently and systematically utilize iterative solvers in the primal update. Numerical simulation studies on a utility maximization problem are presented that illustrate the proposed method.

==> tex/fixpoint.tex <==
To implement the Algorithm~\ref{alg:inexactAL} on a fixed point platform, we need to decide the precision of data and number of iterations required to achieve a user-specified accuracy level, the data range to avoid overflow. In this section, we will discuss these issues. We will assume the binary scaling is applied and signed data is used. Generalization to other scaling techniques should be intuitive.

\subsection{Basics of fixed-point arithmetics}
\label{subsec:basics_fixpoint}
The fixed-point data type has properties: the fractional length $fl$, the word length $wl$ and related arithmetic rules.

The precision of fixed-point data is defined as the maximum error level of the fixed-point data representing a real number. Suppose no overflow happens, the precision of data is determined by the fractional length $fl$ and the chosen rounding scheme. Consider rounding a real number to its nearest fixed-point quantized number, for any scalar $\beta \in \mathbb{R}$ and its fixed point representation $fi(\beta)$, the precision of data is $|\beta - fi(\beta)| \leq 2^{fl + 1}$. Furthermore, for any $v\in \mathbb{R}^n$, $\|v - fi(v)\| \leq \sqrt{n}2^{-(fl+1)}$. And for any $M \in \mathbb{R}^{m \times n}$, we have $\|M - fi(M)\|_{\infty} \leq n2^{-(fl+1)}$.

Next we describe errors introduced in the fixed point arithmetics. Suppose no overflow happens, addition and subtraction between the same fixed-point data type has no error. However, to guarantee a multiplication of two fixed-point scalars, $\beta$ and $\gamma$, in full precision, we need to have the result $fi(\beta\gamma)$ to be of the word length $wl_\beta + wl_\gamma - 1$, where $fi(\beta\gamma)$ means the result of conducting fixed-point multiplication between $\beta$ and $\gamma$. As more multiplicatoins are done, the word length of the stored data explodes. In the following context, we avoid this issue by first conducting multiplication in full precision and then casting the result to designed fixed-point data type, assuming that no overflow happens during the casting. Under this condition, for any $v, u \in \mathbb{R}^n$, $|v^Tu - fi(v^Tu)| \leq n2^{-(fl+1)}$. For any $M \in \mathbb{R}^{m \times n}$ and $v \in \mathbb{R}^n$, we have $\|Mv - fi(Mv)\| \leq \sqrt{m}n2^{-(fl+1)}$.

The data range of fixed-point data is the range of real numbers fixed-point data can represent within the designed precision without overflow happening. The data range is determined by the length of integer bits $wl - fl -1$. We subtract additional 1 bit from the word length for the signedness bit. Signed fixed-point data type with word length $wl$ and fractional length $fl$ can represent data within the interval $[-2^{wl-fl-2}-(1-2^{-fl}), 2^{wl-fl-2}-2^{-fl}]$.

\subsection{An example of the problem}
\label{subsec:example_pb}
To decide how to choose $fl$ and $wl$ to satisfy the Assumption~$\ref{assum:bound_var}$, we need to specific the problem formulation, the algorithm we use to solve the minimization problem at step 2 in the Algorithm~\ref{alg:inexactAL} and some implementation details.

Let us consider a MPC problem:
\begin{equation}
	\label{pb:mpc}
	\begin{split}
		\min & \sum_{t=0}^{N-1}[\frac{1}{2}x_t^TQ_tx_t + \frac{1}{2}u_t^TR_tu_t] + \frac{1}{2}x_N^TQ_Nx_N \\
		\text{s.t. } & x_{t+1} = Ax_t + Bu_t, t = 0,1,\cdots,N-1 \\
		& l_x \leq x_t \leq u_x, t = 0,1,\cdots, N \\
		& l_u \leq u_t \leq u_u, t= 0,1,\cdots, N-1 \\
		& x_0 = b_0
	\end{split}
\end{equation}

For readability, we write the MPC problem~(\ref{pb:mpc}) in a simplified version comparable to the problem~(\ref{pb:problem}):
\begin{equation}
	\label{pb:sim_mpc}
	\begin{split}
	\min & \frac{1}{2}x^THx \\
	\text{s.t. } & Ax = b \\
	& l \leq x \leq u
	\end{split}
\end{equation}
where $x \in \mathbb{R}^n$ is a stacked vector of state vectors $x_t$ and control inputs $u_t$, $H \in \mathbb{R}^{n \times n}$ is a matrix containing energy/cost matrices $Q_t, R_t$ and $Q_N$. $A \in \mathbb{R}^{p \times n}$ is a matrix containing system dynamics matrices $A$ and $B$. $b \in \mathbb{R}^p$ contains the initial state $b_0$. $l$ and $u$ are stacked vectors containing the bounds $l_x, u_x, l_u$ and $u_u$. We also denote the set $\mathcal{X} = \{ x | l \leq x \leq u \}$. We make below assumption about the problem~(\ref{pb:sim_mpc}):

\begin{assumption}
	\label{assum:mpc}
	The parameters in the problem~(\ref{pb:sim_mpc}), $H, A, b, l, u$, can be exactly represented using fixed-point data.
\end{assumption}

For simplicity of implementation, we use the same fixed-point data type to represent all the variables during the Algorithm~\ref{alg:inexactAL}. That is, all the variables have $fl$ fractional bits and $wl$ total bits.

First, we discuss how to solve the minimization problem at step 2 in Algorithm~{\ref{alg:inexactAL}} on a fixed-point platform. Considering the problem (\ref{pb:sim_mpc}), this minimization problem is formulated below: for a multiplier $\lambda_k$ at iteration $k$,

\begin{equation}
	\label{pb:inner_problem}
	\begin{split}
	\min & \frac{1}{2}x^THx + \langle \lambda_k, Ax - b \rangle + \frac{\rho}{2}\|Ax - b\|^2 \\
	\text{s.t. } & x \in \mathcal{X}
	\end{split}
\end{equation}

This problem has no closed form solution due to the constraint, thus we need to apply iterative methods. Since the constraint is a box constraint, which is simple to conduct projection onto, we can apply projected gradient method to solve this problem. Denote $k_{in}$ as the iteration number in the projected gradient method, the operation at each inner iteration is shown below:
\begin{equation}
	\label{eq:oper_inner}
	x_{k_{in} + 1} = \Pi_{\mathcal{X}}[x_{k_{in}} - \frac{1}{L_p}((H + \rho A^T A)x_{k_{in}}  + A^T\lambda_k - \rho A^Tb)]
\end{equation}

where $L_p$ is the Lipschtiz constant of the gradient of the objective function in (\ref{pb:inner_problem}) and $L_p = \sigma_{max}(H + \rho A^TA)$, that is, the largest singular value of the matrix $H + \rho A^TA$.

We can calculate terms $M_1 = \frac{1}{L_p}(H + \rho A^TA)$, $M_2 = \frac{1}{L_p}A^T$ and $V_1 = \frac{\rho}{L_p}A^Tb$ on a more precise platform, e.g. a floating-point platform, and then using their fixed-point representation to run the step (\ref{eq:oper_inner}) as below:

\begin{equation}
	\label{eq:oper_inner_fixpoint}
	x_{k_{in} + 1} = \Pi_{\mathcal{X}}[x_{k_{in}} - fi(fi(M_1)x_{k_{in}})  - fi(fi(M_2)\lambda_k) + fi(V_1)]	
\end{equation}

Fixed-point operation (\ref{eq:oper_inner_fixpoint}) can be seen as an erroneous operation of (\ref{eq:oper_inner}) as below:

\begin{equation}
	\label{eq:oper_inner_err}
	x_{k_{in} + 1} = \Pi_{\mathcal{X}}[x_{k_{in}} - \frac{1}{L_p}((H + \rho A^T A)x_{k_{in}} + A^T\lambda_k - \rho A^Tb + \epsilon_{gp})]	
\end{equation}

where by comparing the equivalent expression (\ref{eq:oper_inner_fixpoint}) and (\ref{eq:oper_inner_err}), we get that:

\begin{equation}
	\label{eq:mag_err_gp}
	\begin{split}
	\|\epsilon_{gp}\| &= L_p\|fi(fi(M_1)x_{k_{in}}) - M_1x_{k_{in}} + fi(fi(M_2)\lambda_k) \\ &\quad \quad \quad \quad \quad \quad \quad \quad \quad \quad - M_2\lambda_k + (V_1 - fi(V_1))\| \\
	& \leq L_p(\|fi(fi(M_1)x_{k_{in}}) - M_1x_{k_{in}}\| \\ &+ \|fi(fi(M_2)\lambda_k) - M_2\lambda_k\| + \|(V_1 - fi(V_1))\|) \\	
	\end{split}
\end{equation}

where the inequality follows from the triangle inequality. Next let us characterize the upper bound of term $\|fi(fi(M_1)x_{k_{in}}) - M_1x_{k_{in}}\|$:

\begin{equation}
	\label{eq:bound_err_gp_term1}
	\begin{split}
	& \|fi(fi(M_1)x_{k_{in}}) - M_1x_{k_{in}}\| \\
	= & \|fi(fi(M_1)x_{k_{in}}) - fi(M_1)x_{k_{in}} + fi(M_1)x_{k_{in}}  - M_1x_{k_{in}}\| \\
	\leq &\|fi(fi(M_1)x_{k_{in}}) - fi(M_1)x_{k_{in}}\| + \|(fi(M_1) - M_1)x_{k_{in}}\|
	\end{split}
\end{equation}

The inequality above follows from the triangle inequality. Since $fi(M_1) \in \mathbb{R}^{n \times n}$, from the discussion in the subsection~\ref{subsec:basics_fixpoint}, we get $\|fi(fi(M_1)x_{k_{in}}) - fi(M_1)x_{k_{in}}\| \leq \sqrt{n}n2^{-(fl+1)}$. Meanwhile, denoting $x_{\infty}^{max} = \max_{x\in\mathcal{X}}\|x\|_\infty$, we get that $\|(fi(M_1) - M_1)x_{k_{in}}\| \leq \sqrt{n}\|fi(M_1) - M_1\|_\infty x_{\infty}^{max} \leq \sqrt{n}n2^{-(fl+1)}x_{\infty}^{max}$. Combining above two results into the inequality~(\ref{eq:bound_err_gp_term1}), we obtain:
\begin{equation}
	\label{eq:bound_err_gp_term1_final}
	\|fi(fi(M_1)x_{k_{in}}) - M_1x_{k_{in}}\| \leq (1 + x_{\infty}^{max})n^{\frac{3}{2}}2^{-(fl+1)}
\end{equation}

Under the similar reasoning in (\ref{eq:bound_err_gp_term1}) and (\ref{eq:bound_err_gp_term1_final}), we obtain that:
\begin{equation}
	\label{eq:bound_err_gp_term2_final}
	\|fi(fi(M_2)\lambda_k) - M_2\lambda_k\| \leq (1 + \lambda_{\infty}^{max})\sqrt{n}m2^{-(fl+1)}
\end{equation}

where $\lambda_{\infty}^{max} = \max_{\lambda\in D}\|\lambda\|_\infty$ can be loosely bounded by $\frac{G(b)_{max}}{\tilde{\sigma}_{min}(A)}$, the upper bound of $\|\lambda^\star(b)\|$ found in the Section~\ref{sec:bound_multiplier}.

Meanwhile, from the discussion in the Subsection~\ref{subsec:basics_fixpoint}, we have that $\|V_1 - fi(V_1)\| \leq \sqrt{n}2^{-(fl+1)}$. Substituting this result, the upper bound in (\ref{eq:bound_err_gp_term1_final}) and (\ref{eq:bound_err_gp_term2_final}) into the inequality (\ref{eq:mag_err_gp}), we obtain:

\begin{equation}
	\label{eq:mag_err_gp_final}
	\|\epsilon_{gp}\| \leq L_p\sqrt{n}((1 + x_{\infty}^{max})n + (1 + \lambda_{\infty}^{max})m + 1)2^{-(fl+1)}
\end{equation}

Now we find the relationship between the fractional length $fl$ and the error in the gradient when we use projected gradient method to solve the minimization problem at step 2 in the Algorithm~\ref{alg:inexactAL}. We will discuss how to determine $fl$ to achieve the accuracy level $\epsilon_{in}^k$ required at step 2 in the Algorithm~\ref{alg:inexactAL}.

({\color{red} We note here that there are other methods applied to solve the inner minimization problem, e.g. fast gradient method. Error analysis of this method under inexact gradient is available in \cite{devolder2014first}. This method gains more popularity in the current literatures.})

Another operation needed in the Algorithm~\ref{alg:inexactAL} is the step 3, calculating $\lambda_{k+1} = \Pi_{D}[\lambda_k + \frac{1}{L}(A \tilde{x}_k - b)]$ using fixed-point data. Similar to the operation in (\ref{eq:oper_inner}), we calculate $M_3 = \frac{1}{L}A$ and $V_2 = \frac{b}{L}$ before running the algorithm and use their fixed-point representation $fi(M_3)$ and $fi(V_2)$ to implement the algorithm. The actual implementation at the step 3 is below:

\begin{equation}
	\label{eq:oper_outer}
	\lambda_{k+1} = \Pi_{D}[\lambda_k + fi(fi(M_3)\tilde{x}_k) - fi(V_2)]
\end{equation}

Comparing the operation in (\ref{eq:oper_outer}) and the exact operation $\lambda_{k+1} = \Pi_{D}[\lambda_k + \frac{1}{L}(A \tilde{x}_k - b)]$, we can conclude that $\epsilon_{out}^k$ at the step 3 in the Algorithm~\ref{alg:inexactAL} satisfies:

\begin{equation}
	\label{eq:mag_err_outer}
	\|\epsilon_{out}^k\| = L\|fi(fi(M_3)\tilde{x}_k) - M_3\tilde{x}_k + V_2 - fi(V_2)\|
\end{equation}

Using similar reasoning from (\ref{eq:mag_err_gp}) to (\ref{eq:bound_err_gp_term2_final}) to get the bound in (\ref{eq:mag_err_gp_final}), from (\ref{eq:mag_err_outer}) we can obtain:

\begin{equation}
	\label{eq:mag_err_outer_final}
	\|\epsilon_{out}^k\| \leq L\sqrt{m}((1+x_{\infty}^{max})n+ 1)2^{-(fl+1)} 
\end{equation}

\subsection{Resolution of data}
\label{subsec:resol_data}
In this section, we discuss how to determine $fl$ so that the Algorithm~\ref{alg:inexactAL} returns a $\epsilon$-optimal solution $\bar{x}_K$. $\epsilon$ is a user-specified accuracy level. $\epsilon$-optimal solution is defined below:

\begin{definition}
	\label{def:optimal_sol}
	We define $\bar{x}_K$ is an $\epsilon$-optimal solution if $\bar{x}_K$ satisfies:
	\begin{equation*}
		|f(\bar{x}_K) - f(x^\star)| \leq \epsilon \text{, and } \|r(\bar{x}_K\| \leq \epsilon
	\end{equation*}
\end{definition}

According to Theorem~\ref{thm:primal_opt_feas}, we find that $\epsilon$ consists of two parts: $\frac{\phi^1(\lambda)}{K}$ where $\lambda$ is chosen as in (\ref{eq:primal_opt_1}),(\ref{eq:primal_opt_2}) and (\ref{eq:primal_feas})  respectively, and the steady state error $E$ characterized in (\ref{eq:steady_error}). Asymptotically, the first part diminishes, thus $\epsilon$ is determined by $E$. However, in practical platform, only limited iteration number $K$ is allowed. Thus we will discuss how to choose $fl$ such that $E \leq \frac{\epsilon}{2}$ in this section. In the next section, we will discuss how to choose $K$ large enough so that $\frac{\phi^1(\lambda)}{2K} \leq \frac{\epsilon}{2}$ holds for all choices of $\lambda$ in (\ref{eq:primal_opt_1}),(\ref{eq:primal_opt_2}) and (\ref{eq:primal_feas}).

First, we will discuss how to assign the accuracy bound $B_{out}$ and $B_{in}$ so that $E \leq \frac{\epsilon}{2}$ will be satisfied. Considering the three terms in the steady error $E$ in (\ref{eq:steady_error}), the term $(\frac{4}{L} + 3)B_{out}B_\lambda$ and the term $(\frac{2}{L}+2)(1+\sqrt{2L_p}B_x)\sqrt{B_{in}}$ are more significant than the term $(\frac{1}{2}+\frac{1}{2L})B_{out}^2$. Thus, we let $(\frac{4}{L} + 3)B_{out}B_\lambda \leq \alpha\frac{\epsilon}{2}$ and $(\frac{2}{L}+2)(1+\sqrt{2L_p}B_x)\sqrt{B_{in}} \leq (1-\alpha)\frac{\epsilon}{2}$,
where $\alpha \in (0,1)$ is a weight parameter to balance the accuracy assigned to the outer iteration and the inner minimization problem. ({\color{red} Apparently simply ignoring the term $(\frac{1}{2}+\frac{1}{2L})B_{out}^2$ is not rigorous here. Also, there should be an optimal strategy to assign $\frac{\epsilon}{2}$ among three terms in the steady state error $E$ so that the fractional length $fl$ is minimized.})

Denoting constants $C_1 = (\frac{4}{L} + 3)B_\lambda$ and $C_2 = (\frac{2}{L}+2)(1+\sqrt{2L_p}B_x)$, we have that:

\begin{equation}
	\label{eq:bound_Bout}
	B_{out} \leq \frac{\alpha\epsilon}{2C_1}
\end{equation}
And 
\begin{equation}
	\label{eq:bound_Bin}
	B_{in} \leq (\frac{(1-\alpha)\epsilon}{2C_2})^2
\end{equation}

Denoting $C_3 = L\sqrt{m}((1+x_{\infty}^{max})n+ 1)$, and combining inequalities (\ref{eq:bound_Bout}) and (\ref{eq:mag_err_outer_final}), we obtain the first criteria of choosing $fl$:

\begin{equation}
	\label{eq:first_fl}
	fl \geq -\log(\frac{\alpha\epsilon}{2C_1C_3}) - 1
\end{equation}

where $\log$ denotes logarithm function with base $2$ in the following context unless otherwise specified.

Second, we will discuss how to choose $fl$ so that the criteria at step 2 in the Algorithm~\ref{alg:inexactAL} can be satisfied. For this purpose, we need to characterize the error of the projected gradient method with an inexact gradient information. Let us take the problem~(\ref{pb:inner_problem}) as an example. Denoting the objective function in (\ref{pb:inner_problem}) as $f_{gp}(x)$, the gradient of this objective function as $g_{gp}(x)$, the inexact gradient $\tilde{g}_{gp}(x) = g_{gp}(x) + \epsilon_{gp}$ and the upper bound of $\|\epsilon_{gp}\|$ characterized in (\ref{eq:mag_err_gp_final}) as $B_{gp}$, we directly present two results in \cite{devolder2014first} and \cite{patrinos2015dual}:

\begin{lemma}
	\label{lem:inexact_oracle_gp}
	(\cite{devolder2014first} Section 2.3b) For problem~(\ref{pb:inner_problem}), $\tilde{f}_{gp}(x) = f_{gp}(x) - B_{gp}B_x$ and $\tilde{g}_{gp}(x) = g_{gp}(x) + \epsilon_{gp}$ is a $(\delta_{gp}, L_{gp})$ inexact oracle of the convex function $f_{gp}(x)$, where $\delta_{gp} = 2B_{gp}B_x$ and $L_{gp} = L_p$.
\end{lemma}

\begin{theorem}
	\label{thm:converg_gp}
	(\cite{patrinos2015dual} Theorem 5) For problem~(\ref{pb:inner_problem}), let $\{x_{k_{in}}\}$ be generated by running the iteration described in (\ref{eq:oper_inner_fixpoint})(or equivalently, (\ref{eq:oper_inner_err})), and let $\tilde{f}_{gp}(x)$ and $\tilde{g}_{gp}(x)$ be an $(\delta_{gp}, L_{gp})$ inexact oracle of $f_{gp}(x)$. Define $\bar{x}_{K_{in} + 1} = \frac{1}{K_{in} + 1}\sum_{t=0}^{K_{in}}x_{t}$. Then
	\begin{equation}
		f_{gp}(\bar{x}_{K_{in} + 1}) - f_{gp}^\star \leq \frac{L_{gp}}{2(K_{in}+1)}B_x^2 + \delta_{gp}
	\end{equation}
\end{theorem}

According to Lemma~\ref{lem:inexact_oracle_gp}, Theorem~\ref{thm:primal_opt_feas} and the upper bound of $\|\epsilon_{gp}\|$ in (\ref{eq:mag_err_gp_final}), we get that:

\begin{equation}
	\label{eq:bound_delta_gp}
	\delta_{gp} = 2B_xL_p\sqrt{n}((1 + x_{\infty}^{max})n + (1 + \lambda_{\infty}^{max})m + 1)2^{-(fl+1)}
\end{equation}

To satisfy the accuracy requirement $\epsilon_{in}^k$ at the step 2 in the Algorithm~\ref{alg:inexactAL}, we need to choose $fl$ and $K_{in}$ to satisfy $\frac{L_{gp}}{2(K_{in}+1)}B_x^2 \leq \frac{\epsilon_{in}^k}{2}$ and $\delta_{gp} \leq \frac{\epsilon_{in}^k}{2}$. We will leave the choice of $K_{in}$ to the next subsection. The criteria $\delta_{gp} \leq \frac{\epsilon_{in}^k}{2}$ gives us the first lower bound of $fl$. Denoting a constant $C_4 = L_p\sqrt{n}((1 + x_{\infty}^{max})n + (1 + \lambda_{\infty}^{max})m + 1)$, then combing $\delta_{gp} \leq \frac{\epsilon_{in}^k}{2}$, (\ref{eq:bound_Bin}) and (\ref{eq:bound_delta_gp}), we get:

\begin{equation}
	\label{eq:second_fl}
	fl \geq -\log(\frac{(1-\alpha)^2\epsilon^2}{16B_xC_2^2C_4}) - 1
\end{equation}

Combining the result in (\ref{eq:first_fl}) and (\ref{eq:second_fl}), we conclude that the fractional length should be chosen such that $fl = \lceil \max\{-\log(\frac{\alpha\epsilon}{2C_1C_3}) - 1, -\log(\frac{(1-\alpha)^2\epsilon^2}{16B_xC_2^2C_4}) - 1\} \rceil$, where $\lceil \beta \rceil$ means ceiling operation, that is, taking the nearest integer larger than $\beta$.

\subsection{Iteration complexity certification}
\label{subsec:iter_complexity}
In this section, we will discuss the choice of inner iteration number $K_{in}$ and outer iteration number $K$ so that an $\epsilon$-optimal solution $\bar{x}_K$ can be achieved.

As discussed before (\ref{eq:second_fl}), $K_{in}$ should be chosen such that $\epsilon_{in}^k$ is achieved when solving the minimization problem at step 2 in the Algorithm~\ref{alg:inexactAL}. When $\delta_{gp} \leq \frac{\epsilon_{in}^2}{2}$, $K_{in}$ needs to satisfy $\frac{L_{gp}}{2(K_{in}+1)}B_x^2 \leq \frac{\epsilon_{in}^k}{2}$. According to Lemma~\ref{lem:inexact_oracle_gp}, $L_{gp} = L_p$. Recalling the bound of $B_{in}$ in (\ref{eq:bound_Bin}), we get:

\begin{equation}
	\label{eq:bound_Kin}
	K_{in} \geq \frac{4L_pB_x^2C_2^2}{(1-\alpha)^2\epsilon^2} - 1	
\end{equation}

Thus $K_{in}$ is chosen to be $K_{in} = \lceil \frac{4L_pB_x^2C_2^2}{(1-\alpha)^2\epsilon^2} - 1 \rceil$.

As discussed after the Definition~(\ref{def:optimal_sol}), the outer iteration number $K$ needs to be chosen such that $\frac{\phi^1(\lambda)}{2K} \leq \frac{\epsilon}{2}$ is satisfied for all choices of $\lambda$ in the (\ref{eq:primal_opt_1}),(\ref{eq:primal_opt_2}) and (\ref{eq:primal_feas}).

Denoting $\phi_{max}^1 = \max\{ \phi^1(0), \phi^1(2\lambda^\star), \phi^1(\lambda^\star + \frac{r(\bar{x}_K)}{\|r(\bar{x}_K)\|}\}$, then it is simple to see that $K$ needs to satisfy:

\begin{equation}
	\label{eq:bound_Kout}
	K \geq \frac{\phi_{max}^1}{\epsilon}
\end{equation}

Thus $K$ is chosen to be $K = \lceil \frac{\phi_{max}^1}{\epsilon} \rceil$.

\subsection{Data Range}
\label{subsec:data_range}
In this section, we will discuss the choice of word length $wl$ so that overflow will not happen during the iterations of the Algorithm~\ref{alg:inexactAL}.

Denoting the word length of $x$ to be $wl_x$, and recalling the operation on $x_{k_{in}}$ iterated in the Algorithm~\ref{alg:inexactAL}, (\ref{eq:oper_inner_fixpoint}), we conclude that for operations on $x_{k_{in}}$ not to overflow, we need $wl_x$ to satisfy:

\begin{equation*}
	\begin{split}
	2^{wl_x - fl - 2} - 2^{-fl} \geq & x_\infty^{max} + \|fi(M_1)\|_\infty x_\infty^{max} \\ &+ \|fi(M_2)\|_\infty \lambda_{\infty}^{max} + \|fi(V_1)\|_\infty	
	\end{split}
\end{equation*}

Denoting $C_5 = x_\infty^{max} + \|fi(M_1)\|_\infty x_\infty^{max} + \|fi(M_2)\|_\infty \lambda_{\infty}^{max} + \|fi(V_1)\|_\infty + 2^{-fl}$, then we have that:

\begin{equation}
	\label{eq:data_range_x}
	wl_x \geq \log(C_5) + fl + 2
\end{equation}

Denoting the word length of $\lambda$ to be $wl_\lambda$, and recalling the operation on $\lambda_k$, (\ref{eq:oper_outer}), we conclude that for operations on $\lambda_k$ not to overflow, we need $wl_\lambda$ to satisfy:

\begin{equation*}
	2^{wl_\lambda - fl - 2} - 2^{-fl} \geq \|\lambda\|_\infty^{max} + \|fi(M_3)\|_\infty x_\infty^{max} + \|fi(V_2)\|_\infty
\end{equation*}

Denoting $C_6 =  \|\lambda\|_\infty^{max} + \|fi(M_3)\|_\infty x_\infty^{max} + \|fi(V_2)\|_\infty + 2^{-fl}$, then we have that:

\begin{equation}
	\label{eq:data_range_lambda}
	wl_\lambda \geq \log(C_6) + fl + 2
\end{equation}

Since we use the same word length for variable $x$ and $\lambda$, we conclude that the word length $wl$ should satisfy:

\begin{equation}
	\label{eq:data_range}
	wl \geq \max\{ \log(C_5) + fl + 2,  \log(C_6) + fl + 2 \}
\end{equation}

Thus we choose the word length to be $wl = \lceil \max\{ \log(C_5) + fl + 2,  \log(C_6) + fl + 2 \} \rceil$ so that overflow will not happen during the Algorithm~\ref{alg:inexactAL}.


==> tex/multiplier.tex <==
We continue the discussion in the Remark~\ref{remark:D_delta}. To let the set $D_\delta$ satisfy conditions in the Remark~\ref{remark:D_delta}, we need the radium in each dimension of the set $D_\delta$ to be at least $r_\delta = \max\{\|\lambda^\star\|_{\infty}, \|\lambda^\star\|_{\infty}+\|\epsilon_{out}^k\|_{\infty}, 0, 2\|\lambda^\star\|_{\infty}, \|\lambda^\star\|_{\infty} + 1\}$. In this case, the bound in (\ref{eq:bound_multiplier}) $B_\lambda = 2\sqrt{p}r_\delta$, where $p$ is the dimension of the multiplier. Thus, to decide $B_\lambda$ is essentially characterizing $\|\lambda^\star\|_{\infty}$. However, we note here that determining $\|\lambda^\star\|_{\infty}$ is also important to decide the set $D$ to conduct projection operation in step 3 in the Algorithm~\ref{alg:inexactAL}.

In implementations on the fixed-point platform, parameters in the Problem~(\ref{pb:problem}) usually cannot be pre-determined. For example, in a MPC problem, parameter $b$ contains the initial state information and usually is determined online. In this case, to decide sets $D$ and $D_\delta$, we need to consider the parameterized optimization below:

\begin{equation}
	\label{pb:param_problem}
	\begin{split}
	x(b) = & \arg \min f(x) \\
	& s.t. \quad Ax = b \\
	& \quad \quad \quad x \in \mathcal{X}
	\end{split}
\end{equation}

where $b \in \mathcal{B}$ and the primal optimal solution $x(b)$ and optimal multiplier $\lambda^\star(b)$ are both parameterized by $b$. In order to determine sets $D$ and $D_\delta$ to accommadate every possible $b \in \mathcal{B}$, we actually need to characterize $\max_{b \in \mathcal{B}} \|\lambda^\star(b)\|_{\infty}$.

Computable bounds for the inequality multiplier exist in \cite{nedic2009approximate} and \cite{patrinos2014accelerated}. \cite{nedic2009approximate} presents a bound that can be calcualted by finding a feasible point satisfying the Slater condtion. This bound is simply for the optimizaiton problem with fixed parameter. \cite{patrinos2014accelerated} provides a uniform bound for the optimization problem with the parameter belonging to a set. In the contrast, there are no results on the bound of equality multiplier that is easy to implement. \cite{mangasarian1985computable} presents the bound for multipliers of both constraints for a nonlinear problem. This scheme needs to find a local solution of the problem. In convex case, a local solution is also a global solution. Thus to find bound of the multiplier reduces to solve the optimization problem. \cite{richter2011towards} proposes another method to find a uniform bound of the equality multiplier for optimization problem parameter belong to a set. However, the compuation of this bound is only trackable for small size problem.

We propose a new method to characterize the bound of the multiplier for equalities based on our previous results in \cite{lee2017complexity}.

\begin{theorem}
	\label{thm:soomin}
	(Bound of multiplier \cite{lee2017complexity}) For problem~(\ref{pb:problem}), let Assumption~\ref{assum:prob_form} and \ref{assum:strong_dual} hold. Let $\|s(x)\| \leq G$ where $s(x)$ is the subdifferential of $f(x)$ and $x \in \mathcal{X}$. Then
	\begin{equation}
		\label{eq:soomin}
		\|\lambda^\star\| \leq \frac{G}{\tilde{\sigma}_{min}(A)}
	\end{equation}
	where $\tilde{\sigma}_{min}(A)$ is the smallest nonzero singular value of $A$.
\end{theorem}

Now let us consider the parameterized problem~(\ref{pb:param_problem}), in Theorem~\ref{thm:soomin}, $G$ can actually be upper bounded by the maximum value of below problem:

\begin{equation}
	\label{pb:bound_multiplier}
	\begin{split}
	& \max_{x, b} \|\nabla f(x)\|^2 \\
	& \text{s.t.} \quad Ax = b \\
	& \quad \quad x \in \mathcal{X}, \quad b \in \mathcal{B}
	\end{split}
\end{equation}

Denote the maximum value of problem~(\ref{pb:bound_multiplier}) as $G^2(b)_{max}$. Then we obtain:

\begin{equation}
	\label{eq:bound_multiplier_final}
	\max_{b\in\mathcal{B}} \|\lambda^\star(b)\| \leq \frac{G(b)_{max}}{\tilde{\sigma}_{min}(A)}
\end{equation}

It is simple to see that bound in (\ref{eq:bound_multiplier_final}) can serve as a loose upper bound of $\max_{b \in \mathcal{B}} \|\lambda^\star(b)\|_{\infty}$.

Under some specific problem formulations, problem~(\ref{pb:bound_multiplier}) can be solved in reasonable time. For example, in an MPC problem with quadratic objective and linear time-invariant dynamics, and furthermore $\mathcal{X}$ and $\mathcal{B}$ are polyhedral, problem~(\ref{pb:bound_multiplier}) falls into the class of nonconvex quadratic programming problems. Such problem with moderate dimension can be solved by commerical package, e.g. CPLEX in reasonable time.

({\color{red} I don't understand part of the proof in \cite{lee2017complexity} Theorem 3. How to get (27)? Also we may need additional assumption about differentiability of $f(x)$ to make problem~\ref{pb:bound_multiplier} make sense.})

